Black Hole Mergers and Unstable Circular Orbits

We describe recent numerical simulations of the merger of a class of equal mass, non-spinning, eccentric binary black hole systems in general relativity. We show that with appropriate fine-tuning of the initial conditions to a region of parameter space we denote the threshold of immediate merger, the binary enters a phase of close interaction in a near-circular orbit, stays there for an amount of time proportional to logarithmic distance from the threshold in parameter space, then either separates or merges to form a single Kerr black hole. To gain a better understanding of this phenomena we study an analogous problem in the evolution of equatorial geodesics about a central Kerr black hole. A similar threshold of capture exists for appropriate classes of initial conditions, and tuning to threshold the geodesics approach one of the unstable circular geodesics of the Kerr spacetime. Remarkably, with a natural mapping of the parameters of the geodesic to that of the equal mass system, the scaling exponent describing the whirl phase of each system turns out to be quite similar. Armed with this lone piece of evidence that an approximate correspondence might exist between near-threshold evolution of geodesics and generic binary mergers, we illustrate how this information can be used to estimate the cross section and energy emitted in the ultra relativistic black hole scattering problem. This could eventually be of use in providing estimates for the related problem of parton collisions at the Large Hadron Collider in extra dimension scenarios where black holes are produced.

==> response_to_referees <==
Please thank the referees on our behalf for reading through the
manuscript in such detail and making useful and constructive suggestions.
Below we outline responses to particular questions, either describing
the changes we made in the paper to answer the questions, or explaining
why we decided not to make changes.

First referee's report
----------------------

This paper points out an interesting analogy between critical phenomena for
comparable mass binaries simulated in numerical relativity, and geodesics of
particles in a Kerr black hole background.

The critical phenomena investigated in this paper could shed light on some
theoretical implications of numerical simulations of black hole binaries. I
found the paper very interesting and thought-provoking, and I strongly
encourage the authors to continue their investigation.

However, at this stage some aspects of the proposed analogy seem to be based
on circumstantial evidence. On several occasions, I had the impression that
some claims in this paper are little more than informed speculations.

  (*) Author's response: Here we respond to the above statement and several
      statements below made by the referee regarding the "circumstantial evidence",
      "weak evidence", that certain claims are "dangerous", etc. First,
      we agree with the referee that much of what is in the paper is speculation,
      however, we feel that we have been very up-front and honest about that
      in the paper. Second, we are in the process of trying to see if the
      proposed analogy between certain aspects of geodesic motion
      apply beyond the equal mass problem, however these simulations are very
      expensive, and it will be years before a few extra data-points 
      supporting or disproving the conjecture is available. Furthermore, we
      believe this is a very interesting problem, if only from
      a theoretical perspective, and thus it is important to present it in
      the scientific literature. Third, simply presenting the raw numerical
      data without interpretation would be "safe", but this is rather
      puzzling behavior for the equal mass binary problem, and immediately
      begs the question "what's going on?". At a first glance the
      behavior didn't make any sense to us, and it was in trying to answer
      this exact question that we found the geodesic analog. As the referee
      pointed out this might just be a coincidence in one example,
      but from our point of view the important thing is it provides
      an explanation that intuitively makes sense. If it turns out
      to be wrong then we are back to square one, i.e. what's going on.
      If not, there are interesting consequences, some of which we speculate
      about in the paper.

      We have gone through the paper and changed a few words and sentences
      to make sure it's absolutely clear when we are speculating, though
      again we believe we were already reasonably careful about doing that 
      to begin with.

I found a number of typos and inaccuracies that the authors should address
before publication. They are listed below.

Page 1, right column, line 9:

"based on coordinate separation, the binaries are orbiting within what would
be the innermost stable circular geodesic of a Kerr spacetime with angular
momentum equal to that of the black hole that forms in the merger case"

This is the kind of "circumstantial evidence" I mentioned above.

I have two main concerns about this statement.

First of all, the statement is based on the (unjustified) assumption of a
quantitative correspondence between harmonic coordinates and the
Boyer-Lindquist coordinates of the geodesic analogue.

Ref.[13] showed that harmonic coordinates seem to work very well in SOME
applications, as pointed out in footnote 1. However, I think it is very
dangerous to attach physical meaning to the coordinate separation of
equal-mass binaries, and even more dangerous to extrapolate their meaning to
extreme mass-ratio binaries.

Secondly, the existence of innermost stable circular orbits is a very
questionable concept (to say the least) whenever the binary's mass ratio is
not extremal.

Things get even worse in higher dimensions. The authors are well aware that,
to be astrophysically relevant, the critical behavior found in this paper
would require an unreasonable amount of fine tuning, and they propose to look
for critical phenomena in multidimensional black hole production in
TeV-gravity scenarios. Unfortunately, in higher dimensional black hole
spacetimes there are no stable circular orbits.

For non-rotating black holes, the non-existence of stable circular orbits was
pointed out in the very first paper on the subject:

F.~R.~Tangherlini, Nuovo Cim.\ {\bf 27}, 636 (1963).

For rotating (Myers-Perry) black holes this was shown, for example, in:

V.~P.~Frolov and D.~Stojkovic, Phys.\ Rev.\ D {\bf 68}, 064011 (2003)
[arXiv:gr-qc/0301016].

See also

V.~Cardoso and S.~Yoshida, JHEP {\bf 0507}, 009 (2005)
[arXiv:hep-th/0502206]

for some implications of the non-existence of stable circular orbits in these
spacetimes.

Therefore, claiming that critical phenomena may be relevant at the LHC based
on an extension of the geodesic analogy to higher dimensions is very
dangerous. Fortunately many arguments in this paper do not seem to rely on the
existence of STABLE circular orbits, but this caveat is certainly worth
mentioning. In my opinion the geodesic analogy should be explored more
carefully, especially in the higher-dimensional scenario. I would also
recommend to rephrase many of the statements in this paper to take into
account the possibility that the proposed "geodesic analogy" is not valid.
One such statement is on page 1, bottom right ("The close analogy [...]
kinetic energy-dominated regime").

=> Author's response: see (*) above, and in response to questions
   about higher dimensional scenarios, it is crucial that there
   are *unstable* circular orbits for this qualitative behavior to
   possibly exist in any particular black hole spacetime regardless
   of the dimension. So things do certainly not get worse in higher
   dimensions. We have added a statement clarifying this in the paper, and
   added the above references.
   Note that another misperception about these results that
   many people seem to immediately assume is that this is "critical phenomena"
   in any formal sense. Only in the most colloquial sense of the
   phrase is this critical phenomena, and never in the text do we call
   it that.

Page 7, bottom right, text referring to Fig.8:

Like I said before, I would not trust very much the identification of
coordinates. For this reason, I am afraid that the "reasonable" agreement of
the spin parameters (given the large error bars in the numerical simulation)
may be little more than a coincidence. In my opinion, this paragraph is really
stretching the geodesic analogy. (There is also a small typo: the "0" in "r0"
should be subscript).

The same remark applies to the last two paragraphs in the caption of
Fig. 8. Once again, I would not exclude the possibility that the "rather
remarkable" agreement really is a coincidence. The idea of defining an
"effective initial eccentricity" from the geodesic analogue is interesting.
However, given the weak evidence for the correspondence between the two
problems, using the correspondence to get information on the "full" binary
black hole problem is dangerous (unless, of course, this definition can be
shown to be in quantitative agreement with other estimates of the orbital
eccentricity in the simulations).

Footnote 5 on page 9:

A small remark: one does not necessarily need two precessing spins to have
precession of the orbital plane. For example, generic orbits of non-spinning
particles in a Kerr background have three different orbital frequencies
(Omega_r, Omega_theta and Omega_phi), and only in very special cases do they
lie on a plane.

=> Author's response: we have clarified the footnote

It is not clear to me whether the "bisection" argument of Fig. 9 (and the
related discussion in Section VA) would apply in the general, non-planar case.

I must admit that I found the whole discussion in Section VA quite
confusing. I am not fully convinced of the validity of the conjecture that all
of the kinetic energy could be radiated in GWs "at threshold", modulo the
limits imposed by the area theorem. In fact, this conjecture may even be
false, and I have a feeling that it should be false in "realistic" settings.

I am inclined to believe that in practice there will always be a finite number
of orbits "around threshold" that can be used to radiate GWs. To increase the
number of "zoom-whirl" orbits, one would need to inject an amount of energy in
GWs which almost exactly balances the energy radiated in GWs during the
zoom-whirl. I think (but I have no proof of this statement) that this would
require a large amount of fine tuning. Perhaps calculations of the radiated GW
energy from zoom-whirl orbits in a Kerr background, where the orbits are tuned
to threshold, could help quantify the amount of fine tuning which is needed in
the geodesic case. In the binary black hole case, I am afraid that a
quantitative estimate of this fine tuning could be hopeless because of
computational limitations.

Also, the remark that "when slowly lowering a small mass to a black hole it is
theoretically possible to extract all of the rest mass energy" is slightly
academic and somehow misleading. The statement is only true for the idealized
case of a point-particle being lowered adiabatically, i.e. ignoring GW
emission. As soon as one includes gravitational radiation, or considers that
the particle's size cannot be smaller than (say) the particle's Compton
wavelenght, this statement is not true: see eg. Eq.(15) in

J.~D.~Bekenstein, Phys.\ Rev.\ D {\bf 7}, 2333 (1973).

Similar practical limitations could also apply to the conjecture that "all the
kinetic energy will be converted to GWs at threshold", limiting the amount of
radiatable energy well below the bound imposed by the area theorem. In any
case, this problem deserves further investigation.

=> Author's response: We have removed the statement about a test mass,
   as it is irrelevant to the discussion.

Besides these points of principle, below I list some minor remarks.

In Fig. 6 and 7 it is mentioned that the unstable circular orbit approached in
the zoom-whirl phase has (respectively) r<4 and r>4, which is consistent with
the orbit being unbound/bound. This statement is correct, if slightly
counterintuitive. A very brief reminder on the properties of circular orbits
in the Schwarzschild spacetime (eg., the relation between orbital energy and
radius) may be helpful.

=> Author's response: It is easiest to understand turning points of the
   motion and how they related to eccentricities in terms of the effective
   potential of the orbit ... we think it will be too much of a
   digression to review that in this paper, so instead we have added a reference
   to a standard textbook treatment of this (MTW).

In the caption of Fig.9, it is said that only one black hole is shown because
the coordinates of the second black hole (x2,y2)=-m1/m2(x1,y1). I don't see
the reason why this Newtonian relation should apply in GR. Also, it is not
completely clear from the text if this plot refers to geodesic integrations or
actual numerical trajectories (and there are no labels on the x- and y-axes).

=> Author's response: We have removed the parenthetical comment about where 
   the coordinates of the second BH would be. This figure is a schematic 
   illustration, so refers to neither specific numerical trajectories nor 
   geodesic integrations, which is why we didn't add any labels. 

In Section VB (second paragraph), spins or electric charges of the black holes
are said to be "irrelevant" for sufficiently large Gamma. I am not aware of
any quantitative justification of this statement, and some reference would
help.

=> Author's response: We have added a statement explaining this ...
   essentially, the electric charge and spin of a black hole
   is invariant under a Lorentz boost, and so the ratio of spin or electromagnetic
   energy relative to kinetic energy goes to zero in the limit. Said
   another way, the leading order description of the problem becomes
   closer to the collision of gravitational shock waves, which represent
   all the kinetic energy of the boost.

Footnote 6 on page 10 claims that "current experiments suggest the Planck
scale cannot be very far below maximum LHC energies". "Below" should probably
read "above". In any case, unless I am missing something, I don't see how
current experiments can say anything about energy regimes which have not been
probed yet. Once again, some reference would help.

=> Author's response: Since current accelerators such as the Tevatron
   can reach energies up to 1 TeV, and have not seen anything
   that would require Planck scale physics, it is safe to conclude
   that the "true" Planck scale is above 1TeV. Thus, for the LHC
   to see BH's, the true Planck scale must be some where between
   1 and 7 Tev roughly, which is not very far below maximum LHC
   energies (7TeV).

Below Eq.(34): how sensitive are the estimates to the approximation that
n(\bar b=2)=0? Also: in integrating (35) to get (37), why was it assumed that
all the energy is radiated at threshold, instead of assuming (consistently
with the discussion in the text) that the area-theorem bound applies?

=> Author's response: The estimates are not particularly sensitive
   to the approximation that E(n(\bar b=2)) is exactly zero rather
   than some small number. For this problem we are in the kinetic
   energy dominated regime, and the area theorem will give something
   like E_{max} = 1 - .71/Gamma ~ 1 in the large Lorentz-Gamma limit.

Page 11, right column, last paragraph: the cross section is first said to be
well approximated by (pi b*^2)/4; then it is stated that for b*\sim 2E, the
effective cross section for measurable energy loss is 4\pi E^2. Is this a
typo, or am I missing something?

=> Author's reponse: the "cross section for black hole production" (i.e. merger)
   is (pi b*^2)/4; however for impact parameters greater than this even
   though a merger doesn't result, a significant amount of energy could
   still be "lost" to gravitational waves. Thus if energy loss is the
   signal for non-standard model physics, then the "effective cross section
   for measurable energy loss" is larger than the black hole production
   cross section ... roughly 4 times larger with this particular estimate.

At the very end, it is mentioned that studies of geodesic scattering and
head-on collisions in higher dimensions could be used to provide information
in the higher dimensional case. One such study can be found in

E.~Berti, M.~Cavaglia and L.~Gualtieri, Phys.\ Rev.\ D {\bf 69}, 124011 (2004)
[arXiv:hep-th/0309203].

=> Author's response: we have added a reference to this paper.

A couple of recommendations to improve presentation: I think that Eq.(31)
should be presented just below Eq.(14), to make it clear that omega is a
constant for circular orbits. Furthermore, before Eq.(17), an explanation of
the reason why \delta r_0 should be proportional to p-p* would be helpful.

=> Author's response: We have moved equation (31) to just after equation (14),
   and explicitly now call it $\omega_0$, to differentiate it from a couple
   of places in equations following where the general, non-constant $\omega$ can 
   be used.

I conclude with a list of typos I spotted:

In notes 1, 2, 3, 5, 6 the first letter is lowercase, and punctuation is
missing.

Page 3, three lines from end of Sec. IIC: "m=m1+m2 is the total..mass", not
masses.

Page 3, Sec. IIIA, line 7: this phenomena -> this phenomenon.

Above Eq.(15): I think \delta_r(t) should read \delta r(t)

Below Eq.(16): have been complete -> have been completed

Page 8, right column, 8 lines from end: bizzare -> bizarre

Page 9, top right: I believe that "apoaps" should really be "apoapsis"

Summary and conclusions: three lines from end of first paragraph,
as many 20-30 orbits -> as many as 20-30 orbits

While this estimate is useful, I am not convinced of its reliability, because
it assumes (without compelling evidence) that the area theorem, and not some
other process, is limiting GW emission at threshold. 

=> Author's response: We have fixed all the above typos.


Second referee's report
-----------------------

This paper discusses a very interesting and intriguing aspect of
evolutions of binary black hole spacetimes, the existence of
"a threshold of merger" in one-parameter families of initial
configurations. By fine-tuning the corresponding initial parameter, the
black holes approach a state of close interaction and remain in that state
for a period of time which increases exponentially as a function of
the distance of the parameter from a critical value, before
eventually merging or separating. This behavior is analogous in
various regards to the well-known "critical phenomena".
The paper continues by demonstrating a strong analogy to a similar
behavior observed for geodesics in Kerr spacetimes. Finally, the
authors draw conclusions regarding the expected energy emission
and cross section in collision experiments to be performed in future
with the Large Hadron Collider (LHC).

The paper contains a wealth of interesting information, to quite
some extent on previously hardly charted territory. As a somewhat
natural consequence, several statements made in this work are based on
circumstantial evidence, rather than rigorous arguments. While the
paper should definitely be published eventually, clarification is
needed on some issues, in my opinion. I also found a small number of simple
typos which I list at the end of this report.

01) On page 2L, at the beginning of Sec.II, ten references are given
on the GHG field equations. This is about 30% of the total number
of references and thus makes the citations a bit unbalanced. I will
give some examples in the following items, where additional
references (on other topics) would be helpful.

=> Author's response: We have added several additional references
   to hopefully make it more balanced.

02) Page 3R, Sec.III A: I believe a table summarizing the most important
parameters of the individual simulations would be helpful. It would
be nice if this table also includes the ADM masses or (equivalently)
binding energies.

=> Author's response: We have described the relevant parameters
   in detail in the second paragraph of sec. III.A, and
   don't believe it will add too much to the presentation to repeat
   this information in a table. With regards to the ADM mass,
   because a certain percentage (~15%) of the scalar field
   does not fall into the black holes and escapes to infinity,
   the ADM mass is not such a useful quantity here. In principle one could try
   to measure a binding energy as ADM mass minus escaped scalar field energy
   minus apparent horizon masses, but we did not save enough scalar field
   information to compute this from exisiting data, and furthermore it will
   be difficult to integrate the scalar field energy with sufficient accuracy
   to recover what is probably a very small binding energy.

03) Page 4L: Is there a particular reason, why no value of (k*-k)
was evolved using different resolutions? Even if the convergence
thus obtained is not quite satisfactory, it would help estimating
the resulting errors. (cf. item 05 below).

=> Author's response: The key piece of information we wanted
   to extract from the simulations for this paper was the 
   scaling exponent gamma, and in this case we did estimate the
   errors using convergence testing. Though given the exponential
   sensitiviy of the solution to (k-k*) this requires doing a set
   of independent threshold searches at different resolutions,
   and then doing convergence testing of the desired property
   of the set of solutions (gamma in this case). More "traditional"
   convergence tests with similar data were shown in
   F. Pretorius, {\em Class. Quant. Grav.} {\bf 23}, S529 (2006),
   and for brevity we didn't reproduce those results here.

04) Table 1: If possible without significant additional work, could
the (initial) coordinate radii of the apparent horizons be included for
comparison with the resolutions?

=> Author's response: Instead of adding another column (the value
   is essentially the same for all resolutions) we have added a line
   in the text of the caption to the table with this information.

05) Page 5R: Here the authors discuss the impact, gravitational
wave emission might (should?) have on the behavior of the
black holes near the unstable circular orbit. I am also
surprised by the fact that such an impact is hardly present in
the numerical studies. I believe that for resolving this question,
more systematic convergence analysis is required (cf. item 03).
While I do not demand that the authors add such a study to the
present manuscript (because it would be computationally very
expensive), I believe, a statement such as "In order to
resolve this question, it will be important in future work to
perform systematic convergence analysis..." should be added in some
place.

=> Author's response: What we were really trying to emphasize
   in this paragraph is how counter-intuitive, at a first glance,
   this behavior in the equal mass problem is. I.e., in the
   geodesic case this an unstable configuration, and so one
   would intuitively expect that this behavior won't even manifest
   in the full problem. However it does, and at *each* resolution
   we studied, with all signs that we are converging to this.
   And thus, as we tried to argue in
   Section V.A., the resolution to the "problem" is understanding
   that this kind of behavior is not only possible in the equal mass case,
   but "natural" and in hindsight expected. Note that we are in a very different
   regime from the qausi-circular inspiral picture where radiation
   reaction steadily shrinks orbits. 
   A more thorough convergence test would add higher resolution simulation points
   to Fig.1 (this figure captures the essense of the behavior,
   and looking at constraints, energies, waveforms, etc. will not
   help in clarifying the issue), though we believe that the three
   resolutions shown in Fig.1 already gives rather compelling evidence
   that this is "real", and not sourced by numerical error.

06) Page 5R: Fig.5: It would be nice to add a plot of the energy
flux as a function of time. In particular, it would be interesting
to compare the energy fluxes for simulations as the initial
parameter is fine-tuned towards criticality. I would be most interested
in the behavior of the flux amplitudes as we get closer to the
threshold. From the good agreement with the quadrupole calculation,
I expect that the amplitude will not depend strongly on the fine-tuning,
but it would be encouraging to have this information in a figure.

=> Author's response: We have added a figure showing the energy
   flux from several simulations.

07) Page 6L, text after Eq.(16): As I understand, $\omega$ is assumed
as constant in this argument. This is made clearer further below
in the discussion of Eq.(31). It would help to either move Eq.(31)
to this location or, at least point to it.

=> Author's response:  We have moved equation (31) to just after equation (14),
   and explicitly now call it $\omega_0$, to differentiate it from a couple
   of places in equations below where the general, non-constant $\omega$ can
   be used.

08) Page 7L, very end of Sec.IV A: The authors argue that the
difference between the radial coordinates $r$ and $R_0$ is not
significant because of more important difficulties arising
out of the comparison with the full numerical simulations. Is it
possible to estimate the error resulting out of using $r$ and
$R_0$ which might provide a lower limit of the uncertainties?

=> Author's response: expression (31) is without error ... whether
   it is written in terms of $r$ or $R_0$, it will still give
   the same numerical value. The point is if we want to compare
   it to a numerical simulation we need to estimate a radius from
   the numerical simulation, and this is where the uncertainty
   will come in, not in any differences between Boyer-Lindquist
   r and proper circumference R_0. We have simplified this paragraph
   a bit to hopefully avoid any confusion.

09) Page 7R: last line of regular text: The agreement between $a=0.5$
and $a=0.7$ is not quite convincing, especially if one takes
into account that the ellipse in Fig.8 might well be larger due
to numerical errors. I am thus a bit uncomfortable with the
phrase "which is close to".

=> Author's response: we have changed "which is close to" to 
   "which is not too far from". Perhaps this phrasing, though
   similar to what was before, conveys better that we are not
   claiming they are the same. Note though that given the area
   of allowed gamma's and r_0's on the plot spanned by the geodesics,
   and that there is no a-priori reason to expect such a linear 
   relationship of n vs ln|k-k*| in the full problem, let alone
   that the slope is anywhere near the geodesic values, we
   think the agreement, though not exact, is remarkably close.

10) Page 8, Figs.6, 7: The authors stress the bound (unbound) nature
of the orbits as the unstable circular orbit has r < 4 (r > 4).
I believe this to be attributed to the energy of the particle on
the corresponding orbits. It would help for clarity if the energy
would be given explicitly or pointed to in the form of a reference.

    Author's response: We have added a reference to the MTW 
    description of particle motion, which containts a fairly
    detailed accounting of the kinds of orbits, energies, etc.

11) Page 9L: Caption of Fig.8, last sentence: I do not see, how eccentricity
suddenly enters the game, considering that the discussion in Sec.IV A
has focused on circular unstable orbits. Most certainly I am missing
something here.

=> Author's response: the *exact* unstable circular orbits don't 
   have an eccentricity in the traditional sense of the word, 
   but for each point on gamma(r0) corresponding to some
   r0>r0_min(a) [r0_min(a=0)=4], if you perturb it by
   an *infinitesimal* amount, it will "unravel" to a zoom-whirl
   type orbit (for the case it doesn't fall into the black hole)
   with a unique, *finite* eccentricity ... as for example in Fig. 7.
   Thus the rather bizaare situation that there are orbits which 
   remain arbitrarily close to the given circular orbit for an 
   arbitrary long amount of time but which have finite and sizeable
   eccentricities. For (r0<r0_min(a)) the perturbed orbit
   will be unbound.


12) Page 9R, last sentence of first paragraph: I am confused by the statement
"will fade, for ever sooner after separating the binaries will merge."

=> Author's response: we have re-written that sentence as follows
   to hopefully make it clearer: "Of course,
   approaching this point the notion of an ``immediate merger''
   will become ill-defined, for ever sooner after separating the binaries will
   merge and thus it will become impossible to differentiate
   between prompt merger and separation."

13) Page 9R: The statement "for when slowly lowering a small mass to a black
hole it is theoretically possible to extract all of the rest mass
energy..." should be supported by a reference.

=> Author's response: we have removed this remark in response to a comment
   by the first referee.

14) Page 9R: End of second paragraph: The authors state that "it should
be possible for all the kinetic energy to be emitted as gravitational
waves at the threshold". I am not quite convinced, that the argument
extends to extreme velocities where the the increased mass of the
system might induce formation of a common apparent horizon at a
much earlier stage than in the "slower" systems studied.

=> Author's response: this is a conjecture on our part, and 
   the alternative suggested by the referee is certainly a possibility.
   To make it more clear that we aren't claiming anything with
   certainty we have changed the "it should be..." to "it may be...".

15) Page 10R: The statement that for sufficiently large boosts, spin
and charge of the black holes become negligible does not seem
obvious to me. I could well imagine a large boost amplifying effects
due to spin/charge. If there are arguments in the literature on this
point, it would be worth adding references, but I am not aware of
any such studies.

=> Author's response: We have added a statement explaining our reasoning ...
   essentially, the electric charge and spin of a black hole
   is an invariant under a Lorentz boost, and so the ratio of spin or electromagnetic
   energy relative to kinetic energy goes to zero in the limit. Said
   another way, the leading order description of the problem becomes
   closer to the collision of gravitational shock waves, which represent
   all the kinetic energy of the boost. 

16) Page 11L, After Eq.(37): "For boundary conditions we have assumed all
the energy is radiated for b=1". Does "all the energy" really mean E, i.e.
the total ADM mass of the spacetime?

=> Author's reponse: yes, and the error in this assumption, assuming
   area-theorem bounds hold, will be of order 1/Gamma, where Gamma
   is the Lorentz Gamma factor, and so can be arbitrarily small
   for large boosts.

17) Page 11L, second paragraph after Eq.(37): "though for values of b
such that E_r(b) < 0.29 (37) is still valid." I do not see, how
E_r(b) can still be valid in that regime even though we have used an
unrealistic boundary condition. I would expect the boundary condition
to affect the function E_r(b) in an adverse manner for all values of b.

=> Author's reponse: we have reworded this statement to say 
   "...such that $\Ebar(\bbar)<\approx.29$ (\ref{eb}) is still a very 
   good approximation." Changing the b.c. at b=1 has very little
   affect on the shape of the curve except in a region close to b=1,
   but so close that the result would be imperceptable from the
   curve plotted in the top part of Figure 10. The boundary
   conditions at \bar{b}=0 and \bar{b}=2 have a much more noticable
   effect on the curve.

18) Page 11R, last paragraph: The authors briefly discuss the effect of
the boundary condition E_r(b=2) = 0 which might lead to an
underestimation of the radiated energy. I have the impression, that
the other boundary condition E_r(b=1) = 1 might lead to an overestimation.
This should be commented upon.

=> Author's response: In the large Gamma limit we think E_r(b=1) = 1 is
   not an over-estimation, as conjectured in the previous section.
   Again, this is not something we can prove, but we believe we
   have made it sufficiently clear that many of these calculations
   are based on speculation.

19) Page 12R: Fig. 10 (lower panel). In the caption, it is stated that
E_r approaches a step function as a->1. From the curves in the figure,
it appears that the solid curve is closest to a step function. But this
curve has the smallest value of a. Is it possible that the labels of
the curves are reversed?

=> Author's response: we have clarified that the curve approaches
   the "unit step function $\Theta(\bbar/2)$". The curve
   with the smallest a might be approximated (ignoring the spiky-bit)
   by $0.16 \Theta(\bbar)$, but in the limit a->1 that curve
   exactly becomes $\Theta(\bbar/2)$

20) In the Summary and Conclusions section, a few statements are initially
put in a rather strong way, but then called into question (again in
a rather strong fashion) in the final paragraph. This section would
be more homogenous if the statements are initially phrased in a
milder form and the final paragraph focuses on the outlook
towards future work. The statements I have in mind are

- 3rd paragraph: "that such a threshold must exist for generic..."
The authors themselves have noted a few possible caveats
in their argument in Sec.V A.

=> Author's response: we have tried to tone done the langauge a bit
   throughout the manuscript, making it clearer when we are speculating
   and when we have some evidence for what we say.

- 2nd line on Page 13: "At threshold it is possible that essentially
all...". This is not really a result, as far as I can see, but a
(reasonable) conjecture.

=> Author's response: have changed the word "possible" to "conceivable"

Having listed these points, I would like to emphasize that I have enjoyed
reading the manuscript and found it very stimulating in many areas.

I conclude with a brief list of minor typos:

- Caption of table I: line 2: "were each resolution..."
"where each resolution..."

- Caption of Fig.5: 4th line from bottom: "non-merger cased..."
"non-merger case..."

- 3rd line above Eq.(14): "number of orbits increase as the..."
"number of orbits increases as the..."

- Just before Eq.(15): the $\delta r$ has the r as subscript

- 4th line after Eq.(16): "have been complete..."
"have been completed..."

- Page 7R, 1st line: "Fig.'s"
"Figs."

- Page 7R, 4th line from bottom: "value of ($r0,..."
"value of ($r_0,..."

- Page 9R, 2nd line: "every lenthier..."
"ever lengthier..."

- Eq.(38): Subscript on right hand side is "qaud" instead of "quad" 

=> Author's response: we fixed all the above typos, spelling errors, etc.

